Performance comparison of timing-based anomaly detectors for Controller Area Network: a reproducible study

This work presents an experimental evaluation of the detection performance of eight different algorithms for anomaly detection on the Controller Area Network (CAN) bus of modern vehicles based on the analysis of the timing or frequency of CAN messages. This work solves the current limitations of related scientific literature, that is based on private dataset, lacks of open implementations, and detailed description of the detection algorithms. These drawback prevent the reproducibility of published results, and makes it impossible to compare a novel proposal against related work, thus hindering the advancement of science. This paper solves these issues by publicly releasing implementations, labeled datasets and by describing an unbiased experimental comparisons.

==> sections/algorithms.tex <==
% \section{Timing-based anomaly detectors}
% \label{s:detectors}
% In the following sections we describe the timing/frequency-based detection algorithms used for the comparison (Section~\ref{ss:algorithms}) and the threat model considered for the experimental evaluation (Section~\ref{ss:threat_model}). 

% \subsection{Timing-based anomaly detectors}
% \label{ss:algorithms}
% In this section we describe the anomaly detectors considered for the experimental evaluation presented in this work. For readability purpose, we associate each algorithm with a particular label composed by the last name of the first authors and the last two digits of the publication year.

% \subsubsection{Otsuka14}
% \label{ss:alg:otsuka}
% % 2 righe intro
% In the work presented in~\cite{Otsuka2014CANSecurity}, the authors designed an anomaly detection algorithm that uses a delayed-decision cycle detection method to detect and prevents spoofing attacks. 
% % come funziona
% The rationale of the algorithm is that data frames are transmitted at a constant cycle designed as $T$, so in case of a spoofing attack, the reception cycle of the attacked data frames is shorter than the designed one. When an ECU receives a data frame with the same CAN ID of the previous data frame and a reception cycle minor of $T$ (plus a margin $B$), the ECU holds the data frame until $T$ is passed. If in the meanwhile that data frame is withheld the ECU receives another data frame with the same CAN ID, the ECU determines that a spoofing attack must have occurred and the data frames are not processed. The algorithm then does not detect the attack immediately and waits for the arrival of $T$ to determine that spoofing attacks have occurred.
% % come è stato testato dagli autori
% They measured the reception cycle for each CAN ID for 10 seconds using data frames collected from an actual car during normal operation. Then they selected as the target
% data of spoofing attacks CAN ID $I$ (due to the relatively stable reception cycle) and $J$ (due to the non relatively reception cycle). The attack was examined using two patterns:
% \begin{enumerate}
%     \item constant cycle: send data frames at a constant cycle of 10ms;
%     \item sliding cycle: send data frames with sliding cycle, which increases of 0.1ms per data frame.
% \end{enumerate}
% % metriche usate dagli autori per capire i risultati
% Finally, they collected the results in terms of False Positive Rate (FPR) and False Negative Rate (FNR).
% % con chi è stato comparato
% This algorithm was compared with previous works~\cite{muter2010structured,van2011canauth,matsumoto2012method} in terms of amount of changes in the ECUs, quality of security features, processing load, and required design information.
% \todo{si può dire numerical?} No numerical detection results were reported.

% \subsubsection{Taylor15}
% \label{ss:alg:taylor}
% In the work presented in~\cite{Taylor2015Frequency}, the authors designed an anomaly detection algorithms for the detection of anomalies based on inter-packet timing over a sliding window. In particular, the algorithm presented in \Taylor uses test values over consecutive CAN flows. Each test value is evaluated as a $t-$test comparing the time difference mean with its historical values. The algorithm then uses the test values for the evaluation of the anomaly score (defined as the log sum) over a sequence of scores, to identify anomalies in the CAN communication. 
% This algorithm is tested against the injection and the removal of CAN messages with different attack duration, ranging from $100$ milliseconds to $1$ second. For the message injection attack and for each duration, the injected packed is inserted once, five, and time times its average rate. The detection performance are presented by means of the Receiver Operating Characteristics (ROC) and the Area Under Curve (AUC) measure. The authors not compared the algorithm with previous works but only with a One-Class Support Vector Machine classifier trained on the same data. 

% \subsubsection{Gmiden16}
% \label{ss:alg:gmiden}
% % 2 righe intro
% In the work presented in~\cite{Gmiden2016Detection}, the authors designed a lightweight intrusion detection algorithm against malicious injected messages, but they do not consider DoS.
% % come funziona
% The proposed IDS in \Gmiden is based on an anomaly-based approach, which makes a frequency analysis to detect attacks in real-time. The IDS checks the arrival time of each data frame and calculates the time interval of the arrival message compared
% to the last message with the same CAN ID. If the interval message is less than half the normal one, an alert will be lifted.
% % come è stato testato dagli autori
% They didn't test the algorithm with real data and proposed only a theoretically analysis of an attack against the cruise control system,
% % metriche usate dagli autori per capire i risultati
% so we don't have any performance evaluation of the algorithm.
% % con chi è stato comparato
% The authors compared the proposed algorithm with~\cite{nilsson2008efficient} and~\cite{lin2012cyber} in terms of compatibility with the existing CAN protocol, and with cryptography-based methods such as~\cite{larson2008approach,lin2012cyber}, and~\cite{miller2014survey} in terms of cost of implementation. 

% \subsubsection{Song16}
% \label{ss:alg:song}
% % 2 righe intro
% In the work presented in~\cite{Song2016Intervals}, the authors presented a hybrid intrusion detection system against message injection, DoS attacks, and anomalies.
% % come funziona
% The proposed algorithms can be considered as a combination of two with the first part in common. When a new message appears on CAN bus, the IDS checks the CAN ID and computes the time interval from the arrival time of the latest message with the same CAN ID. Then the IDS is split into two checks:
% \begin{itemize}
%     \item If the interval of a new message is shorter than normal, then the message is classified as an injected message. In particular, they propose to mark a message as malicious if the interval is half of the normal;
%     \item if the time intervals of the latest messages in a row are less than 0.2 milliseconds, then DoS attack score increased by 1 per message. The IDS classify an event as a DoS attack if the score is larger than a given threshold.
% \end{itemize}
% % come è stato testato dagli autori
% To test the algorithm, they captured 40 minutes of messages from the CAN bus using an actual car and injected messages for 5-10s randomly for each attack. The attacks are injection of messages of a single CAN ID, injection of messages with multiple CAN ID, and DoS.
% In particular, for single and multiple CAN IDs, they injected messages with double, quintuple, and decuple faster rates than the origin cycle. For DoS attack, they injected about 2000 messages per second and tested a threshold of 1,2,3, and 5.
% In the test, they used samples of 1 minute.
% % metriche usate dagli autori per capire i risultati
% The results are reported in terms of detection accuracy,
% % con chi è stato comparato
% but the algorithm was not compared with previous works.

% \subsubsection{Moore17}
% \label{ss:alg:moore}
% % 2 righe intro
% In the work presented in~\cite{Moore2017Frequency}, the authors
% propose a signal-frequency-based CAN-bus anomaly detection algorithm, that does not require a priori system-specific knowledge, able to detect sustained regular-frequency signal injection attacks.
% % come funziona
% They defined with $\Delta_1=t_1-t_0, ..., \Delta_n=t_n-t_{n-1}$ the wait times between two messages with the same PID received at time $t_i$. Then, they found the maximum observed error from expectation as $m=max_i\left\|\Delta_i - \mu\right\|$ with $\mu=\sum\nolimits_{i}^{}\Delta_i/n$.
% Messages are flagged if the time between signals
% differs in absolute value from the expected wait time by more than $\alpha=m+0.15\cdot\mu$, and an alert is triggered if there are three flagged wait times consecutively.
% % come è stato testato dagli autori
% They tested the algorithm using three attacks during two normal vehicle operation models, which are engine on and off respectively. In the first two attacks, they injected regular-frequency messages into the CAN bus at a rate high enough to suppress the ambient signal also sent regularly by the car. The third is a DoS attack. The model was trained observing five seconds of clean CAN data and tested against a dataset with 29-45s of consecutive attacks surrounded by non-attack data.
% % metriche usate dagli autori per capire i risultati
% They reported the detection results in terms of true positive rate, false positive rate, and false detection rate.
% % con chi è stato comparato
% \Moore was not compared with previous works.

% \subsubsection{Stabili19}
% \label{ss:alg:stabili}
% In the work described in~\cite{Stabili2019Missing}, the authors designed an anomaly detection algorithm for the detection of missing messages from CAN communication. In particular, the algorithm presented in \Stabili evaluates the cycle-time ($ct$) of each CAN ID to built its detection model.
% In the detection phase, the cycle time is used in conjunction with a configuration parameter $k$ (defined in the validation process for each ID) to detect missing messages from the CAN bus. A message with a particular ID is considered missing if it is not send on the CAN bus for a minimum period of $ct*k$ milliseconds from the last message with the same CAN ID.
% This algorithm is tested against two similar attack scenarios, the \textit{ECU shutdown} attack (in which messages with a particular ID are removed from the CAN for a period of time that ranges from $10$ to $120$ milliseconds)  and the \textit{ECU inhibition} attack (in which all messages with a particular ID are removed from the CAN bus). The detection performance are presented by means of the $F$-measure and compared with other detection algorithms, despite only \Moore is used for the comparison with similar works.


% \section{Threat Model}
% \label{s:threat_model}
% In this work we define a threat model that is built on the threat models considered in the original works of the tested detection algorithms~\cite{Otsuka2014CANSecurity,Taylor2015Frequency,Gmiden2016Detection,Song2016Intervals,Moore2017Frequency,Stabili2019Missing}. The threat model is composed by two different attack scenarios, the \textit{message injection} and the \textit{message removal} attacks.


% \subsubsection{Message injection}
% \label{sss:message_injection}
% % Message injection 
% %   --> Replay di messaggi in base al loro cycle time e non a caso ma con frequenze diverse
% %   --> Solo di messaggi ciclici e validi (per i quali è possibile costruire un detection model)
% %   --> 
% The message injection attack scenario is used to inject messages on the CAN bus to subvert its normal behavior, by exploiting modern drive-by-wires capabilities such as brake-by-wire or steer-by-wire. 
% The message injection attack scenarios comprises different attacks, such as the \textit{replay attack}, in which a message already seen in the CAN communication is injected at a later time on the network, the \textit{fuzzing attack}, in which messages with malformed values in its fields are injected to study the consequences on the system, and the \textit{denial-of-service}, in which messages with high priority are injected with a high frequency to disrupt the normal CAN communications.
% For the aim of our analysis, we do not focus on either the \textit{fuzzing} and \textit{denial-of-service} for the following reasons:
% \begin{itemize}
%     \item in case of a \textit{fuzzing attack} to the ID field of the CAN data frame, the detection algorithms would fail to detect any ongoing attack since it is not possible to build the detection model for a never observed message;
%     \item the \textit{fuzzing attack} on the data field of the CAN data frame (with a legit message ID) can be considered as a \textit{replay attack} on the same message;
%     \item the \textit{denial-of-service} attack scenario can be analyzed by considering a \textit{replay attack} with a high frequency of injection.
% \end{itemize}
% Hence, for the aforementioned reasons, we focus only on the \textit{replay attack} injection scenario. 
% The replay attack is conducted by injecting on the CAN communication a target message (usually selected after an initial phase of reverse engineering of the values encoded in the payload) with a particular injection frequency. 

% \subsubsection{Removal attack}
% \label{sss:removal}
% The removal attack scenario is used to remove messages from the CAN bus to subvert its normal behavior, preventing the ECUs from receiving data required for their functioning.
% The removal attack scenario is composed by two different attack scenarios, as already presented in~\cite{Stabili2019Missing}: the \textit{ECU shutdown} and the \textit{ECU inhibition} attacks. However, since the only difference between the two attacks is the time of the attack and its duration, which do not impact on the overall performance of the detection algorithms, in this work we only focus on the \textit{ECU inhibition} scenario, in which target messages are completely removed from the CAN bus. 
% % Since the Shutdown attack is a particular scenario of the inhibition attack, for the purposes of this paper we inspect the detection capabilities of the BYOD framework against inhibition attack.
